Checking Temporal Properties of Presburger Counter Systems using Reachability Analysis

Counter systems are a well-known and powerful modeling notation for specifying infinite-state systems. In this paper we target the problem of checking temporal properties of counter systems. We first focus on checking liveness properties only, and propose two semi decision techniques for these properties. Both these techniques return a formula that encodes the set of reachable states of a given system that satisfy a given liveness property. A novel aspect of our techniques is that they use reachability analysis techniques, which are well studied in the literature, as black boxes, and are hence able to compute precise answers on a much wider class of systems than previous approaches for the same problem. Secondly, they compute their results by iterative expansion or contraction, and hence permit an approximate solution to be obtained at any point. We state the formal properties of our techniques, and also provide experimental results using standard benchmarks to show the usefulness of our approaches. Finally, we provide a technique for checking arbitrary CTL temporal properties, which use the liveness property checking techniques mentioned above as black boxes.

==> conclusions.tex <==
Before concluding this paper, we would like to thank Dr A.Finkel, Dr S. Demri and Dr J. Leroux for discussions, suggestions and feedbacks all throughout the 
course of this work.
In this paper, we give two algorithms with different approximation capabilities to answer $\eg$ properties. We show that these algorithms can be incorporated 
in a $\ctl$ framework and can be used to answer $\ctl$ properties on various systems. We empirically evaluate our algorithms on some realistic examples which have been previously analyzed
for reachability. We also prove that we address a class of systems which is significantly larger than the class of systems addressed by Demri et al~\cite{dem2006}.
As a part of the future work we would like to compare to granularity of approximations of the two approaches. We would also like to extend our algorithms to address $\ctl^*$ properties.

==> figure.tex <==
% \begin{tabular}{cc}
\begin{figure}
%\centering
%\begin{multicols}{2}
%\begin{minipage}{.5\textwidth}
%\begin{figure}
\makebox[0.4\textwidth]{
\subfigure[]{\input{grow22.pdf_t}}
}
 \makebox[0.4\textwidth]{
 \subfigure[]{\begin{align*}%\begin{split}
%    \forall i, j \in \Sigma. \, (g_i \wedge f_i) \wedge (g_j \wedge
%     f_j[s^{\prime\prime}/ s^\prime]) \implies \\
%     (s^\prime = s ^{\prime\prime}) \vee ((Y[s^\prime/s] \wedge Y[s^{\prime\prime} / s])\\
%     \vee (Y[s^\prime/ s] \wedge \neg Y[s^{\prime\prime}/ s]) \vee  (\neg Y[s^\prime/ s] \wedge Y[s^{\prime\prime}/ s]))
% %\end{split}
 \end{align*}
}
 }
\caption{$\growtwo$}
\label{over_approx:single_trace2}
\end{figure}
% &
% \end{tabular}
%\end{minipage}
%\end{subfigure}
%\end{columns}
%\end{figure*}

==> global-over-nondet.tex <==
\begin{algorithm}
	\caption{$\computeGlobalOverNondet{M}{\phi}{\enumlabel}$}
	\label{algo:compute-global-over-term}
	\begin{algorithmic}[1]
		\REQUIRE A counter system $M$, A set of states $\phi$ and an enumerator $\enumlabel\in\latticeApprox$.
\ENSURE Returns a formula $\phi_1$ and an enumerator $\approximation \in \latticeApprox$. The enumerator $\approximation$ indicates whether $\phi_1$ is precise or is over-approximation or
under-approximation of the set of states of $M$ that satisfy $\eglobally{\phi}$.

		\STATE $M_1\gets\refineSystem{M}{\phi}$
		\STATE $X=\emptyset, Y= \neg (g_1 \vee g_2 \vee \dots \vee g_n) \, \vee \neg \phi$
		\WHILE{not forcefully terminated}
		% \STATE $\mathit{Flat} \gets$ Generate new $k_1$ number of flattenings.\label{line:gen_flat}
		% \FORALL{$N \in \mathit{Flat}$}
		% \STATE $X\gets X \vee \forall k \geq 0. \prek{N}{\phi}$ \label{line:growX}
		% \STATE $(Y,\mathit{flag})\gets\checkflattening{M_1}{N}{\phi-X}{Y}$
		% \IF {$\mathit{flag}$}\label{line:term-Under}
		% \RETURN $(X,\precise)$
		% \ENDIF
		% \STATE $(X_1,Y_1)\gets \computeGlobalUnderOver{M_1}{\phi}{X}{Y}{k_1}$.
		% \ENDFOR
		\STATE $Y \gets Y \vee \mathit{nonDetStates}$
        \STATE \COMMENT{$\mathit{nonDetStates}$ is a non-deterministically chosen subset of the set of all states that do not satisfy $\eglobally{\phi}$.}

		\STATE $Y\gets \computeGlobalOverNew{M_1}{\phi}{Y}$
		\IF{$Y$ returned above is equal to $Y$ given as argument}
		\RETURN $(\neg Y,\precise)$
		\ENDIF
		\ENDWHILE
		% \STATE $X\gets X \vee \forall k \geq 0. \prek{N}{\phi}$ \label{line:growX}
		% \STATE $\phiBad\gets\getBadStates{M_1}{N}$


		% \STATE $Y \gets Y \vee \neg\phiBad\wedge\neg X$


		\IF{$\enumlabel=\under$}
		\RETURN $(X,\under)$
		\ELSE
		\RETURN$(\neg Y,\overapprox)$
		\ENDIF


		%   \IF{$\enumlabel=\under$} 
		%     \STATE $(\phi_1,\approximation)\gets\computeGlobalUnder{M}{\phi}$
		%     \ELSE
		%       \STATE$(\phi_1,\approximation)\gets\computeGlobalOver{M}{\phi}$
		%      \ENDIF
		%      \RETURN $(\phi_1,\approximation)$.
		%       
	\end{algorithmic}
\end{algorithm}


==> global-under-nondet.tex <==
\begin{algorithm}[t]
	\caption{$\computeGlobalUnderNondet{M}{\phi}{\enumlabel}$}
	\label{algo:compute-global-under-term}
	\begin{algorithmic}[1]
		\REQUIRE A counter system $M$, A set of states $\phi$ and an enumerator $\enumlabel\in\latticeApprox$.
 \ENSURE Returns a formula $\phi_1$ and an enumerator $\approximation \in \latticeApprox$. The enumerator $\approximation$ indicates whether $\phi_1$ is precise or is over-approximation or
under-approximation of the set of states of $M$ that satisfy $\eglobally{\phi}$.


		\STATE $M_1\gets\refineSystem{M}{\phi}$
		%\STATE $X=\emptyset, Y= \neg (g_1 \vee g_2 \vee \dots \vee g_n) \, \vee \neg \phi$.
		\STATE $X=\emptyset$.
		\WHILE{not forcefully terminated}
		\STATE $\mathit{Flat} \gets$  $k_1$ fresh flattenings of $M_1$.\label{line:gen_flat}
		\FORALL{$N \in \mathit{Flat}$}
		\STATE $X\gets X \vee \forall k \geq 0. \prek{N}{\phi}$

        %\STATE $(Y,\mathit{flag})\gets\checkflattening{M_1}{N}{\phi-X-Y}$
        \STATE $(\_,\mathit{flag})\gets\checkflattening{M_1}{N}{\phi-X}$

        \IF {$\mathit{flag}$}
		\RETURN $(X,\precise)$
		\ENDIF
		% \STATE $(X_1,Y_1)\gets \computeGlobalUnderOver{M_1}{\phi}{X}{Y}{k_1}$.
		\ENDFOR
		%\STATE $Y \gets Y \vee
        % \mathit{nonDetStates}$\label{line:under-nondet-grow}
        % \STATE \COMMENT{$\mathit{nonDetStates}$ is a non-deterministically chosen subset of the set of all states that do not satisfy $\eglobally{\phi}$.}
		% \STATE $Y\gets Y\vee\computeGlobalOverNew{M}{\phi}{Y}{k_2}$\label{line:growY}
		% \IF{$Y$ has not changed}\label{line:term-Over}
		% \RETURN $(\phi-Y,\precise)$
		% \ENDIF
		\ENDWHILE
		% \STATE $X\gets X \vee \forall k \geq 0. \prek{N}{\phi}$ \label{line:growX}
		% \STATE $\phiBad\gets\getBadStates{M_1}{N}$


		% \STATE $Y \gets Y \vee \neg\phiBad\wedge\neg X$


		\IF{$\enumlabel=\under$}
		\RETURN $(X,\under)$
		\ELSE
		%\RETURN$(\neg Y,\overapprox)$
        \STATE \emph{Error}
		\ENDIF


		%   \IF{$\enumlabel=\under$} 
		%     \STATE $(\phi_1,\approximation)\gets\computeGlobalUnder{M}{\phi}$
		%     \ELSE
		%       \STATE$(\phi_1,\approximation)\gets\computeGlobalOver{M}{\phi}$
		%      \ENDIF
		%      \RETURN $(\phi_1,\approximation)$.
		%       
	\end{algorithmic}
\end{algorithm}


==> illus_over.tex <==
\subsubsection{Illustration of Over-approximation algorithm}
Consider the example system given in Figure~\ref{fig:example_intro} and the property $\eglobally {(x < 10)}$.
The over-approximation algorithm initializes the set $Y$ to $x \geq 10$  which are the stuck states
in refined system shown in Figure~\ref{fig:example_refinement}. 
In the first iteration of the loop state $(x = 9)$ has its only successor $(x = 10)$ in $Y$ and hence 
will satisfy $grow_1$.
Also, the states $(x >= 5) \wedge (x < 9)$ have only one outgoing trace starting from them
and every such trace ends in state in $x = 9$. Hence states $(x >= 5) \wedge (x < 9)$ satisfy $grow_2$. 
In the next iteration no states satisfy $grow_1$ and $grow_2$ and hence the algorithm will
terminate. It returns the set of reachable states that are not in $Y$. This is the set $(x \geq 0) \wedge (x < 5)$. 

==> implementation.tex <==
\label{ssec:implementation}
Given a counter system $M$ and a set of states $\phi$ our algorithms return a Presburger formula for 
the set of states that satisfy $\eglobally{\phi}$ and indicates the direction of approximation of the 
returned formula with respect to the actual set of states that satisfy the property 
$\eglobally{\phi}$ in the counter system $M$. In our implementation we aim for precise computations and therefore 
we go into non-termination in some cases. But in cases where we terminate we give precise results. Hence we do not 
return any labels in the implementation. We implement our by modifying the tool FAST~\cite{fast}. The modifications done in the 
tool to implement each of the algorithms is 
described in Sections~\ref{ssec:under-approx-implementation} and~\ref{ssec:over-approx-implementation} (Vasanta to fix this ref).

\subsection{Implementation of Algorithm~\ref{algo:under_approx}}
\label{ssec:under-approx-implementation}
Recall that Algorithm~\ref{algo:under_approx} computes a growing under approximation of the set of states that satisfy $\eglobally{\phi}$.
The implementation of this algorithm involves implementation the following three subroutines:\\
\textbf{Generation of flattenings:} Algorithm~\ref{algo:under_approx} first generates a flattenings of increasing lengths. This generation must ensure that the flattenings 
 are explored in a breadth first way. Generating flattenings in a breadth first way will require the storage of all flattenings of the length $i$ before the flattenings of length $i+1$
 are computed. In cases of larger systems we observe that storing these flattenings take a huge amount of memory and therefore we perform several optimizations to reduce the 
 search space of the flattenings being explored. Firstly we remove the transitions whose guards are unsatisfiable after refinement. Then we also remove transitions whose actions 
 result in a state that does not satisfy $\phi$. Even with these optimizations the search space of flattenings remains huge. Therefore we employ a different strategy for exploration.
 Given a length $i$, We first generate flattenings of length $i$ in a depth first way. We then sweep the entire width of the tree of flattenings for that particular depth.
Therefore every flattening of a given depth is explored. This requires only a single flattening to be stored in memory during execution.


 \noindent \textbf{Computing} $\mathbf{\forall k\geq 0.\ \prek{N}{\phi}:}$
As described in Section~\ref{sec:global}, Algorithm~\ref{algo:under_approx} computes $\forall k\geq 0.\ \prek{N}{\phi}$, where $N$
is a flattening of the counter $M_1$ which is a refinement of $M$ wrt $\phi$. To compute $\forall k\geq 0.\ \prek{N}{\phi}$ it 
requires a black-box to compute a Presburger Formula for $\prek{M}{\phi}$. The black-box that we use for this purpose is the tool 
FAST~\cite{fast}. FAST being a reachability analysis tool, computes a Presburger formula (in $\vec{s}$) for 
$\exists k \geq 0.\ \prek{N}{\phi}$. This is done by computing a Presburger formula for $\prek{N}{\phi}$ using acceleration 
techniques. We use this formula returned by FAST and append a $``\forall k\geq 0''$ to get the formula for 
$\forall k\geq 0.\ \prek{N}{\phi}$. 


\noindent \textbf {Trace equivalence check :} This check is used as the termination condition in Algorithm~\ref{algo:under_approx}.
This check was provided by Demri et al~\cite{dem2006}. We implement this check in the tool FAST.
%\end{itemize}


==> secAlgo.tex <==
\label{sec:algo}
In this section we sketch our inductive algorithm for finding the set of
states in a counter system that satisfy any given $\ctl$ property.  
%In cases where the algorithm 
%cannot compute the results precisely it approximates the results based on user input (label).
%We start with formally defining syntax of $\ctl$ properties and then describe the intuition behind
%our inductive algorithm.
%
%A $\ctl$ property is used to specify a property that a state and the traces starting from that state should satisfy. 
%Following the idea of Demri et al.\cite{dem2006} we extend the $\mathit{CTL}$ grammar to let Presburger 
%formulas of the form $\phi$ be the basic propositions in the temporal properties. 
%Temporal properties in the \emph{existential normal form} of CTL can be defined by the
%following grammar
%\begin{equation} 
%\psi\ \equiv\ \phi\, |\, \neg\psi\, |\, \psi \vee \psi\,
%  |\, \enext{\psi}\, |\,
%\euntil{\psi}{\psi}\, |\, \eglobally{\psi}
%\label{eqn:enf}
%\end{equation}
%Any $\mathit{CTL}$ formula involving universal path quantifiers has an
%equivalent $\mathit{CTL}$ formula in existential normal form. Therefore, we
%restrict ourselves to formulas in existential normal form. Throughout the report we use $\psi, \psi_i$, etc., to denote temporal
%properties. 
The algorithm takes a counter system $M$, a $\ctl$ temporal
property $\psi$, and an \emph{approximation label} as input. The CTL property
is assumed to be in \emph{existential normal form}, where the main
operators are \textbf{EG}, \textbf{EU} (``exists until''), and \textbf{EX}
(``exists next''). The label, which is from the set
\{$\overapprox$, $\under$, $\precise$\}, specifies the allowed direction of
approximation in case the set of states that satisfy $\psi$ in $M$ cannot
be computed precisely. The algorithm works in two passes.  The first pass
is a top-down pass, where the objective is to identify the allowed
direction of approximation for each sub-property of $\psi$. An interesting
aspect here is that `$\neg$' operators cause the allowed direction of
approximation to get reversed.  In the second pass the set of states that
satisfy each sub-property is computed in a bottom-up manner. \textbf{EU}
and \textbf{EX} properties are fairly straightforward to solve, while
for \textbf{EG} properties one of our algorithms $\computeGlobalUnderName$
or $\computeGlobalOverName$ needs to be used depending on the label
assigned to the operator in the first pass. A
detailed discussion of this algorithm can be found in our technical
report~\cite{tech-report}.

%Consider the example $\ctl$ property $\eglobally{(\euntil{\phi_1}{\neg \eglobally{\phi_2}})}$ where 
%$\phi_1$ and $\phi_2$ are Presburger formulas on counters in input counter system. The
%states satisfying $\phi_1$ and $\phi_2$ can be computed precisely as they are basic propositions.
%Let the input label be $\overapprox$. If the given label for entire property is $\overapprox$
%then the set of states satisfying sub-property $\euntil{\phi_1}{\neg \eglobally{\phi_2}}$ must be 
%either precise or over-approximated. On the other hand if assigned approximation direction for 
%property $\euntil{\phi_1}{\neg \eglobally{\phi_2}}$ is $\overapprox$ the approximation 
%direction for nested property $\eglobally{\phi_2}$ is $\under$. This is due to negation operator applied to
%$\eglobally{\phi_2}$. 
%When the direction of approximation is $\overapprox$ then selected routines can compute either a precise
%or an over-approximated result. Similarly, when direction of approximation is $\under$ the computed
%result can be precise or an under-approximation. But if given label is $\precise$ then
%results have to be computed precisely and inductive algorithm may go
%into non-termination due to non-termination of selected routines.


==> secGlobalOverThmFME.tex <==
\subsection{Theoretical claims}
\label{sec:over_approx_correctness}

We have already argued informally that the algorithm (a) maintains a
growing under-approximation $Y$ of the set of states in $M_1$ that do not
satisfy $\eglobally{\phi}$, and (b) terminates iff $Y$ becomes precisely
equal to this set.

In order to make an intuitive argument about termination we argue
termination of our algorithm on three successive classes, each one wider
than the previous one. The first class is the class of systems $M$ such
that the refined system $M_1$ is flat and such that $\mathit{pre}^*$
queries on it terminate. Any flat system can be seen as a directed acyclic
graph (DAG), whose elements are simple cycles or transitions that are not
part of any cycle. We argue that the algorithm ``processes'' any element
$e$, i.e., identifies all states ``in'' the control-states in $e$ that need
to be added to $Y$, in the immediate subsequent iteration after all
successor elements of $e$ in the DAG have been processed. Intuitively,
$\growone$ is responsible for processing elements that are transitions, and
$\growtwo$ for simple cycles.


The next class is the class of systems $M$ such that the refined system
$M_1$ has a \emph{trace
flattening} wrt $\phiinit$ and such that  $\mathit{pre}^*$ queries on $M_1$
terminate. This is a generalization of the class on which the approach of
Demri et al.~\cite{dem2006} terminates. Our argument for this class is a
simple extension of our argument for flat systems that is based on the
structure of the trace flattening of the system $M_1$ rather than on the
structure of $M_1$ itself.

Our final class is of systems $M$ such that (a) $\mathit{pre}^*$ queries on
the refined system $M_1$ terminate, (b) there exists an integer bound $k$,
and a (finite or infinite) set of flattenings of $M_1$ such that each
flattening $N$ in the set contains at most $k$ simple cycles (each one
involving an
arbitrary number of control states), and such that each trace in $M_1$ that
starts from a state that does not satisfy $\eglobally{\phi}$ is exhibited
by at least one of the flattenings mentioned above. (As it was with the
under-approximation algorithm, this characterization is a sufficient
condition, and does not exhaustively cover all cases on which our algorithm
terminates.) 

We provide a proof sketch of the final claim above, and full proofs of all
other claims  in Appendix~\ref{sec:over_approx_correctness-proof}.

An interesting question that is left to future work is to determine
whether our over-approximation algorithm terminates on
a wider class of systems than our under-approximation algorithm. (The
converse is definitely not true.)

%In this section we state the results that prove that output computed by Algorithm~\ref{algo1} is either precise 
%or an over-approximation of set of states that satisfy the given property $\eglobally{(\phi)}$. The detailed 
%proofs of the lemmas and theorems can be found in our technical report~\cite{techReport}.
%\begin{lemma}
%\label{lemma:invariant}
%A state $s$ is added to $Y$ in Algorithm~\ref{algo1} if and only if all states in $\mathit{post^*(M_1,s)}$ are in $Y$.
%\end{lemma}
%
%\begin{theorem}
%\label{thm:over-approx1}
%Given a counter system $M$ and a CTL temporal formula $\eglobally{(\phi)}$, Presburger formula $Y$ computed 
%in each iteration of the loop in Algorithm \ref{algo1} is an under-approximation of the set of states that \emph{do not} 
%satisfy the formula $\eglobally{(\phi)}$ in $M_1$, where $M_1 = \refineSystem{M}{\phi}$.
%\end{theorem}
%We prove both Lemma~\ref{lemma:invariant} and Theorem~\ref{thm:over-approx1} using mathematical induction on the number 
%of iterations of the loop in Algorithm~\ref{algo1}.
%
%Now we give a theorem that proves that if Algorithm~\ref{algo1} terminates then the computed result is precise.
%\begin{theorem}
%\label{thm:over-approx2}
%Given a counter system $M$ and a CTL temporal formula $\eglobally{(\phi)}$ if 
%Algorithm \ref{algo1} terminates then $Y$ represents the precise set of 
%states that do not satisfy the formula $\eglobally{\phi}$ in $M_1$, where $M_1 = \refineSystem{M}{\phi}$. 
%\end{theorem}
%We prove theorem~\ref{thm:over-approx2} by contradiction. We show that is a state that does not 
%satisfy  $\eglobally{(\phi)}$ is not included in $Y$ then the termination condition of the algorithm will 
%not terminate.
%

%% In this section we state the results that prove that Algorithm~$\computeGlobalOverName$ terminates on a trace flattable system
%% independent of the given property. 
%% %Lemmas~\ref{thm:flat_systems},~\ref{thm:trace_flattable_systems1} and Theorem~\ref{thm:trace_flattable_systems2} 
%% %prove that for any given property of the form $\eglobally{\phi}$ Algorithm~\ref{algo1} terminates if the given input
%% %system $M$ is  trace-flattable systems.

%%  \begin{lemma}
%%  \label{thm:flat_systems}
%%  Given a flat counter system $M$ and any property $\eglobally{\phi}$ Algorithm~$\computeGlobalOverName$ will always terminate.
%%  \end{lemma}
%%  We prove Lemma~\ref{thm:flat_systems} by defining a function $\mathit{order}$ that maps each control state in the
%%  given counter system to an integer. We show that for a flat system there is bound on the maximum $\mathit{order}$
%%  value that can be assigned to any control state. We then show using mathematical induction on $\mathit{order}$
%%  value that the algorithm terminates on all flat counter systems.
 
%%  \begin{lemma}
%%  \label{thm:trace_flattable_systems1}
%%  Given a trace flattable counter system $M$ and a property $\eglobally{\phi}$,
%%  set of states added to $Y$ in $n^{th}$ iteration by Algorithm~$\computeGlobalOverName$ is equal to set of states 
%%  added to $Y$ in $n^{th}$ iteration if input counter system was $M_T$, a trace flattening of $M$.
%%  \end{lemma}
%%  We prove Lemma~\ref{thm:trace_flattable_systems1} using mathematical induction on the number
%%  iterations of the while loop in Algorithm~\ref{algo1}. 
 
%%  \begin{theorem}
%%  \label{thm:trace_flattable_systems2}
%%  Given a trace flattable counter system $M$ a property $\eglobally{\phi}$ Algorithm~$\computeGlobalOverName$ will always terminate.
%%  \end{theorem}
%% Since $M_T$ in statement of Theorem~\ref{thm:trace_flattable_systems1} is flat it follows from 
%% Theorem~\ref{thm:flat_systems} that Algorithm~$\computeGlobalOverName$ will always terminate on $M_T$. Hence 
%% using Theorem~\ref{thm:trace_flattable_systems1} it will always terminate if input system $M$ is  a trace flattable system.

%% The over approximation algorithm terminates whenever there exists a constant $k$ such that 
%% length of all path segments in the given counter system is bounded by $k$. Given a trace flattable
%% system there exists a finite number of path segments in the system and hence the lengths of path
%% segments is bounded by length of longest path segment in the given system. Note that 
%% our characterization includes systems that have infinite number of path segments.
 


==> secGlobalOverThmTR.tex <==
%subsubsection{Correctness, precision and termination characteristics of over- approximation approach:\\}
\label{sec:over_approx_correctness-proof}
In this section we formally state and prove the various theoretical claims about Algorithm~$\computeGlobalOverName$, that were made in Section~\ref{sec:over_approx_correctness}.
\begin{lemma}
\label{lemma:invariant}
A state $\vec{s}$ is added to $Y$ in Algorithm~$\computeGlobalOverName$ if and only if all states in $\mathit{post^*(M_1,\vec{s})}$ are in $Y$.
\end{lemma}
\begin{proof}
We prove that if a state $\vec{s}$ is in $Y$ then all states in $\mathit{post^*(M_1,\vec{s})}$ are in $Y$ by proving
the following statement by induction.\\
$\textbf{P(n)}:$ If a state $\vec{s}$ is added to the set $Y$ in the $n^{th}$ iteration of the loop of Algorithm~$\computeGlobalOverName$
then all the states in $\mathit{post^*(M_1,s)}$  will be added to $Y$ in $i^{th}$ iteration where $i \leq n$.\\
\textbf{Base Case (n = 0):} During initialization the set of states that are added to $Y$ are the set of stuck states. 
Stuck states do not have any successor states so $P(0)$ is trivially true.\\
\textbf{Induction Hypothesis:} Let $P(k)$ be true. We now prove that $P(k+1)$ is true.\\
In any iteration of the loop a state can be added to $Y$ under two conditions represented by formulas $grow_1$ and $grow_2$.

\emph{Case 1 ($grow_1$):} Let $\vec{s}$ be a state that satisfies $grow_1$ and thus all successors of $\vec{s}$ are in $Y$.  
By induction hypothesis all states in $\mathit{post^*(M_1,Z)}$ where
$Z$ represents the set of successors of $\vec{s}$ are already in $Y$. 
Hence all states in $\mathit{post^*(M_1,\vec{s})} = Z  \cup \mathit{post^*(M_1,Z)}$ are already in $Y$.\\

\emph{Case 2 ($grow_2$):} Let  $\vec{s}$ be a state that satisfies $grow_2$. On ignoring states in $Y$ 
there is exactly one trace starting from $\vec{s}$ and this trace ends in a state that satisfies $grow_1$. States the belong to
this trace are the states in $\mathit{post^*(M_1,\vec{s})}$ which have not yet been added to $Y$. Let this trace be
$\vec{s}, \vec{s_1}, \vec{s_2}, \dots, \vec{s_n}$, where $\vec{s_n}$ satisfies $grow_1$. In the $(k+1)^{th}$ iteration of the loop $\vec{s_n}$ will be added to 
$Y$ as it satisfies $grow_1$. For all $1 \leq i < n$, a state $\vec{s_i}$ in the trace will have only one successor $\vec{s_{i+1}}$
not in $Y$. If this is not the case then there are multiple traces starting from $\vec{s_i}$ and also from all states $\vec{s_j}$ where 
$1 \leq j < i$. Also all states in the set \{$\vec{s_1}, \vec{s_2}, \dots, \vec{s_{n-1}}$\} are in $\preStar{M_1}{\vec{s_n}}$ and hence 
$\preStar{M_1}{grow_1}$. Thus all states in the set \{$\vec{s_1},\vec{s_2}, \dots, \vec{s_{n-1}}$\} satisfy the formula $grow_2$ and
will be added to $Y$ in $(k+1)^{th}$ iteration of the loop.  Hence statement $P(k+1)$ holds. 

The proof that if all states in $\mathit{post^*(M_1,\vec{s})}$ are in $Y$, then $\vec{s}$ will be added to $Y$ is trivial
as $\vec{s}$ will satisfy $grow_1$ and hence will be added to $Y$.
\end{proof}

\begin{theorem}
\label{thm:over-approx1}
Given a counter system $M$ and a CTL temporal formula $\eglobally{(\phi)}$, Presburger formula $Y$ computed 
in each iteration of the loop in Algorithm~$\computeGlobalOverName$ is an under-approximation of the set of states that \emph{do not} 
satisfy the formula $\eglobally{(\phi)}$ in $M_1$, where $M_1 = \refineSystem{M}{\phi}$.
\end{theorem}
\begin{proof}
We prove statement $P(n)$ defined below using induction. The proof of the theorem follows from this proof:\\
$\textbf{P(n)}:$ If a state $\vec{s}$ is added to $Y$ in $n^{th}$ iteration of the loop in Algorithm~$\computeGlobalOverName$ then
state $\vec{s}$ does not satisfy $\eglobally{\phi}$.\\
\textbf{Base Case (n=0):} $Y$ is initialized to set of stuck states. A stuck state $\vec{s}$ in $M_1$
does not contain any trace starting starting from it. Hence there is no infinite trace stating from $\vec{s}$ 
in $M_1$ and $\vec{s}$ does not satisfy $\eglobally{\phi}$.\\
\textbf{Induction Hypothesis:} Let $P(n)$ be true for all $n \leq k$. We prove that $P(k+1)$ is true.
Since $P(n)$ for $n \leq k$ is true all states added to $Y$ before $(k+1)^{th}$ iteration of the loop
do not satisfy $\eglobally{\phi}$. If a state $\vec{s}$ has to satisfy $\eglobally{\phi}$
then there must exist a infinite trace starting from $\vec{s}$ and all states on this trace must satisfy 
$\eglobally{\phi}$.
In $(k+1)^{th}$ iteration $\vec{s}$ is added to $Y$ if it satisfies $grow_1$ or $grow_2$. 
To show that $P(k+1)$ is true
we need to show that if a state satisfies $grow_1$ or $grow_2$, then the state does not satisfy 
$\eglobally{\phi}$.

If $\vec{s}$ satisfies $grow_1$, then all successors of $\vec{s}$ are in $Y$, hence all traces starting from $\vec{s}$ contain a 
state that does not satisfy $\eglobally{\phi}$. So if $\vec{s}$ satisfies $grow_1$ it will not satisfy $\eglobally{\phi}$.

If $\vec{s}$ satisfies $grow_2$, then there is only one trace starting from $\vec{s}$ along which states do not satisfy $Y$. 
But by definition of $grow_2$ this trace contains a state that satisfies $grow_1$ and as shown above 
if  a state satisfies $grow_1$ it does not satisfy $\eglobally{\phi}$. 
Thus even along this trace $\vec{s}$ does not satisfy $\eglobally{\phi}$.
Hence, $P(k+1)$ is true. 
\end{proof}

Now we give a theorem that proves that if Algorithm~$\computeGlobalOverName$ terminates then the computed result is precise.
\begin{theorem}
\label{thm:over-approx2}
Given a counter system $M$ and a CTL temporal formula $\eglobally{(\phi)}$,
Algorithm $\computeGlobalOverName$ terminates if and only if $Y$ represents the precise set of 
states that do not satisfy the formula $\eglobally{\phi}$ in $M_1$, where $M_1 = \refineSystem{M}{\phi}$. 
\end{theorem}
\begin{proof}
Theorem~\ref{thm:over-approx1} shows that $Y$ is an under-approximation of set of states that do not satisfy
$\eglobally{\phi}$ in $M_1$. 
To show that $Y$ precisely represents the set of states that do not satisfy $\eglobally{\phi}$ in $M_1$ when
algorithm terminates, we need to show that there does not exist a state $\vec{s}$ such that:
\begin{itemize} 
	\item $\vec{s}$ does not satisfy $\eglobally{\phi}$ 
	\item and $\vec{s}$ has not been included in $Y$
\end{itemize}
We prove by contradiction. Let $\vec{s}$ be a state that does not satisfy $\eglobally{\phi}$ and 
on termination of the algorithm has not been included in $Y$.
Since $\vec{s}$ does not satisfy $\eglobally{\phi}$, all traces starting from $\vec{s}$ in $M_1$ are finite. Now we 
show that if we ignore the states that are already added to $Y$, then along every trace starting from
$\vec{s}$ we reach a state that satisfies $grow_1$. If there exists a state that satisfies $grow_1$ and it has
not been included in $Y$ then loop condition ``$grow_1 \wedge grow_2$ is satisfiable" holds and 
contradicts the fact that the while loop in Algorithm~$\computeGlobalOverName$ terminated thus leading to termination 
of the algorithm.

Let $t = \vec{s_1}, \vec{s_2}, \dots, \vec{s_n}$ be a trace starting from $\vec{s}$ where $\forall i \geq 1.$ $\vec{s_i}$ is not in $Y$.
If $\vec{s_n}$ satisfies $grow_1$ then we have shown that termination condition of loop does not hold. 
If $\vec{s_n}$ does not satisfy $grow_1$ then it has a successor $\vec{s_{n+1}}$ that is not in $Y$ and
we can extend the trace $t$ further. 
This cannot be done infinitely as all traces starting from $\vec{s}$ are finite. So eventually we 
reach a state such that all its successors in $Y$ and hence satisfies $grow_1$. Thus we contradict
that while loop in Algorithm~$\computeGlobalOverName$ terminated.

Hence, if the Algorithm~$\computeGlobalOverName$ terminates then the set $Y$ precisely represents that set of states
that do not satisfy $\eglobally{\phi}$.
\end{proof}

The class of systems for which Algorithm~$\computeGlobalOverName$ terminates is a strict superset of trace-flattable systems.
Lemmas~\ref{thm:flat_systems}, \ref{thm:trace_flattable_systems1} and Theorem~\ref{thm:trace_flattable_systems2} 
prove that for any given property of the form $\eglobally{\phi}$ Algorithm~$\computeGlobalOverName$ terminates on all trace-flattable 
systems.

 \begin{lemma}
 \label{thm:flat_systems}
 Given a flat counter system $M$ and any property $\eglobally{\phi}$ Algorithm~$\computeGlobalOverName$ will always terminate on flat systems
 if the calls to $\mathit{pre^*}$ queries terminate.
 \end{lemma}
 \begin{proof}
 Let $M$  be the given counter system. Let $M_1 =$ $\langle Q, C,\Sigma,\phiinit,G,F\rangle$ be the refinement of
 $M$ with respect to $\phi$. Note that if $M$ is flat then $M_1$ will also be a flat counter system.
 We prove a stronger property that Algorithm~$\computeGlobalOverName$ will terminate on a counter system $M$ for any given property $\eglobally{\phi}$
 if $M_1$ is flat. We define a function $\mathit{order_{M_1}}$ thats maps every control state $q \in Q$ in $M_1$ to a natural number.
 Function $\mathit{order_{M_1}}$ is defined as follows:
 \begin{enumerate}
 	\item $\order{{M_1}}{(q)} = 0$, if there is no outgoing transition from $q$
	\item $\order{{M_1}}{(q)} = 1$, if all successor control states of $q$ have an order 0 
	\item $\order{{M_1}}{(q)} = 1$, if $q$ is in a cycle $c$ and no control state in cycle $c$ has a successor outside cycle $c$
	\item $\order{{M_1}}{(q)} = n$, if $q$ is not part of any cycle, has only one successor control state $q_1$ and $\order{{M_1}}{(q_1)} = n$
	\item $\order{{M_1}}{(q)} = n + 1$, if $q$ is not part of any cycle, $q$ has multiple successor nodes and 
	maximum value of $\mathit{order}$ assigned to any successor node of $q$ is $n$
	\item $\order{{M_1}}{(q)} = n + 1$, if $q$ is part of a cycle $c$
	and $n$ is the maximum value assigned to any node $q_1$ that is not part of the cycle but has a predecessor in cycle $c$. 
	Note that every control state in a cycle will have same value for $\mathit{order}$.
 \end{enumerate}
 
 In a flat counter system all cycles are simple. This leads to a partial order between cycles where 
 the relation between two cycles $c_1$ and $c_2$ is defined
 as $c_1 < c_2$ if there exists a sequence of transitions $t_1, t_2,\dots,t_k$ from a control state $q_1$ in $c_1$ to a control state
 $q_2$ in $c_2$. Due to this partial order between the cycles there exists a maximum value for 
 $\mathit{order}$ that can be assigned to a control state in any flat counter automata.
 
 We prove the following statement using mathematical induction which leads to the proof that Algorithm~$\computeGlobalOverName$ terminates on flat counter systems.\\
  $\textbf{P(n)}:$ All states in a control state $q$ that do not satisfy $\eglobally{\phi}$ 
   will be added to set $Y$ in $\leq n$ iterations 
  of the loop in Algorithm~$\computeGlobalOverName$ where $\order{{M_1}}{(q)} = n$. We assume all $\mathit{pre^*}$ queries terminate
  on the given system.\\
  \textbf{Base Case(n=0):} If $n$ is equal to 0 for a control state $q$, then all states corresponding to $q$ will be stuck states 
  as there is no outgoing transition from $q$. All states in $q$ will be added to $Y$ when $Y$ is initialized.\\
  \textbf{Induction Hypothesis:} Let the statement $P(k)$ be true.  We now prove that statement $P(k+1)$ is true. 
  Let $q$ be a control state such that  $\order{{M_1}}{(q)} = k+1$.
  There are four different cases under which a state $\vec{s}$ that has not been added to $Y$ and is in a control state $q$ 
  will not satisfy $\eglobally{\phi}$.  Note that in all the cases computing states that satisfy $grow_2$ is always decidable
  as all $\mathit{pre^*}$ queries terminate on given system.\\
  
  \emph{Case 1:} Let $q$ be part of a cycle $c$ such that no control state in cycle $c$ has a successor outside cycle $c$. 
  Then any state $\vec{s}$ corresponding to $q$ will have only one trace starting from it. 
  This trace will be formed by taking the cycle multiple times. 
  Either the trace ends in a stuck state $\vec{s_1}$ which has already been added to $Y$ or is infinite. 
  A state with a single finite trace ending is $Y$ will satisfy formula $grow_2$. 
  Hence states in $q$ that do not satisfy $\eglobally{\phi}$ will be added to $Y$ in $(k+1)^{th}$ iteration.\\
  
  \emph{Case 2:}  Let $q$ be a state such that $q$ does not belong to a cycle in $M_1$ and has multiple successor control states. 
  Note that for any successor $q_1$ of $q$ $\order{{M_1}}{(q_1)} \leq k$. 
  A state corresponding to $q$ can be a stuck state in which case it is added to $Y$ on initialization. 
  If there is any successor state of $\vec{s}$ that does not satisfy $\eglobally{\phi}$ then by induction hypothesis 
  it is already added to $Y$. This is because it belongs to a control state $q_1$ which is successor of $q$ and 
  $\order{{M_1}}{(q_1)} \leq k$.
  If all successor states of $\vec{s}$ are in $Y$, then $\vec{s}$ satisfies $grow_1$ by definition and does not satisfy 
  $\eglobally{\phi}$. Hence if $\vec{s}$ does not satisfy $\eglobally{\phi}$ it will be added to $Y$ in $(k +1)^{th}$ iteration of the loop.\\
  
  \emph{Case 3:}  $q$ is part of a cycle $c$ and $\order{{M_1}}{(q)} = (k+1)$.
  Note that for every control state $q_1$ in $c$, $\order{{M_1}}{(q_1)} = (k+1)$.
  On ignoring states already in $Y$ every trace $t$ from state $\vec{s}$ will contain only states in the cycle $c$. 
  If not then the trace will contain a state $\vec{s_{\neg q}}$ not in cycle $c$ and which is not in $Y$. $\vec{s_{\neg c}}$
  belongs to a control state $q_{\neg c}$ such that $\order{{M_1}}{(q_{\neg c})} \leq k$.
  By induction hypothesis $\vec{s_{\neg c}}$ satisfies $\eglobally{\phi}$ otherwise it would have been added to $Y$. Hence
  along this trace $\vec{s}$ will satisfy $\eglobally{\phi}$.
  So on ignoring states in $Y$ any trace $t$ starting from $\vec{s}$ which belongs to control state $q$ in cycle $c$, 
  does not satisfy $\eglobally{\phi}$ and has not been added to $Y$ will satisfy one of the following three subcases.
  
  \begin{enumerate}
  	\item \textbf{All states in $t$ belong to a control state in cycle $c$ and $t$ is  infinite:}
	In this case $\vec{s}$ will satisfy $\eglobally{\phi}$ and we are done.
  	\item \textbf{All states in $t$ belong to a control state in the cycle, $t$ is finite and ends in a stuck state $\vec{s_{ss}}$:}
	If any state $\vec{s}$ in $t$ has a successor outside $t$, that successor must be in 
	a control state outside $c$ (because you cannot have branching while staying within $c$). Let $S$ be the set of all successors of states in $t$
	that are outside $c$. The states in $S$ must all not satisfy $\eglobally{\phi}$
	(otherwise $\vec{s}$ would satisfy $\eglobally{\phi}$). The control states to which the
	states in $S$ belong to all have $\mathit{order} \leq k$. Therefore, all states in 
	$S$ would already have been added to $Y$. Therefore, ignoring states that are
	already in $Y$, $t$ is the only trace starting from $\vec{s}$ and this trace ends in a
	stuck state. Starting from $\vec{s}$ the last state on $t$ which does not belong to 
	$Y$ will satisfy $grow_1$. Therefore, $\vec{s}$ will satisfy $grow_2$ and 
	will be added to $Y$ in the $(k+1)^{th}$ iteration.
	
  	\item \textbf{All states in $t$ belong to a control state in the cycle, $t$ is finite and ends in a state $\vec{s_{c}}$ where
	all successors of $\vec{s_c}$ are already in $Y$:} By argument given in subcase 2, every successor
	of a state $\vec{s_1}$ on $t$ which belongs to a control state outside $c$ will be already in $Y$. Hence
	on ignoring states in $Y$, $t$ is the only trace starting from $\vec{s}$ as there is no branching allowed within cycle $c$.
	Now lets say there is no state $\vec{s_{c}}$ on $t$ such that all its successors are in $Y$, then its either the case that
	$\vec{s}$ has no successors in which case it is stuck state and $t$ is covered in subcase 2 or every state in $Y$ 
	has a successor outside $Y$ which makes $t$ infinite which is covered in subcase 1. Thus $t$ is finite and does
	not satisfy condition of subcase 2 then it will contain a state $\vec{s_{c}}$ such that all successors of $\vec{s_{c}}$ are in $Y$.
	Hence $\vec{s_{c}}$ will satisfy $grow_1$ and $\vec{s}$ will satisfy $grow_2$, and $\vec{s}$ will be added to $Y$ in $(k+1)^{th}$ 
	iteration.
  \end{enumerate}
  
  
  Incase $\vec{s}$ does not satisfy $\eglobally{\phi}$ then it can be either a stuck state 
  in which case it is already added to $Y$ or on ignoring states that have been already 
  added to $Y$, $\vec{s}$ will have only one trace starting from it.
  This trace follows the transitions in the cycle before reaching a state like $\vec{s_2}$ that is in control
  state $q_2$ outside the cycle $c$. 
  Since $\vec{s_2}$ will not satisfy $\eglobally{\phi}$ (otherwise $\vec{s}$ will satisfy $\eglobally{\phi}$) and 
  $\order{{M_1}}{(q_2)} \leq k$ by induction hypothesis $\vec{s_2}$ will be 
  already in $Y$. Hence $\vec{s}$ will satisfy $grow_2$.\\
   
  \emph{Case 4:} Let $q$ be a control states that is not part of any cycle and
  has only one successor control state $q_1$. 
  In such cases $\order{M_1}{(q)} = \order{M_1}{(q_1)} = (k+1)$. 
  There will be a sequence of control states $q, q_1, q_2, \dots, q_l$ such that 
  $\forall i < l.$ $\order{{M_1}}{(q_i)} = (k+1)$, $q_i$ does not belong to any cycle 
  and $q_i$ has a single successor control state $q_(i+1)$. 
  $q_l$ can satisfy one of three conditions: 
  \begin{itemize}
  	\item $q_l$ is part of a cycle and $\order{{M_1}}{(q_l)} = (k+1)$
  	\item $q_l$ is not part of any cycle but has multiple successor control states, $\order{{M_1}}{(q_l)} = (k+1)$, 
  and for any successor $q_j$ of $q_l$ $\order{{M_1}}{(q_j)} \leq k$ 
  	\item $\order{{M_1}}{(q_l)} \leq 0$
  \end{itemize} 
  
  If a state $\vec{s}$ in $q$ does not satisfy $\eglobally{\phi}$ then on ignoring states already added to $Y$, $\vec{s}$ will
  have only one trace starting from it and hence will satisfy $grow_2$. This states in the trace will follow the sequence of control 
  states $q_1, q_2, \dots, q_l$ till either it reaches a stuck state or a state $\vec{s_l}$ in $q_l$. The $\vec{s_l}$ does not satisfy 
  $\eglobally{\phi}$ otherwise $\vec{s}$ will satisfy $\eglobally{\phi}$. If $q_l$ is in cycle then as per case 3 described 
  above $\vec{s_l}$ will satisfy $grow_2$. If $q_l$ is not part of cycle and has multiple successors then $\vec{s_l}$ will
  satisfy $grow_1$ as described in case 2. In both these cases $\vec{s}$ will satisfy $grow_2$ and hence will
  be added to $Y$ in $(k+1)^{th}$ iteration. 
  
 If $\mathit{max}$ is the maximum value of $\mathit{order}$ assigned to any control state in given counter system, then 
 Algorithm~$\computeGlobalOverName$ is guaranteed to terminate in $\leq \mathit{max}$ iterations of the inner loop.
  \end{proof}
 
 \begin{lemma}
 \label{thm:trace_flattable_systems1}
 Given a trace flattable counter system $M$ and a property $\eglobally{\phi}$,
 set of states added to $Y$ in $n^{th}$ iteration by Algorithm~$\computeGlobalOverName$ is equal to set of states 
 added to $Y$ in $n^{th}$ iteration if input counter system was $M_T$, a trace flattening of $M$, under the assumption 
 that the calls to $\mathit{pre^*}$ queries always terminate.
 \end{lemma}
 \begin{proof}
 We prove by induction on $n$.\\
 \textbf{Base Case(n = 0):} Set of stuck states in $M$ and $M_T$ are same as all traces are preserved in $M_T$. 
 Hence $Y$ is initialized to same set in both cases.
 \textbf{Induction Hypothesis:} Let the statement be true for $n \leq k$. We now prove that statement is true for $n = (k+1)$.
 We can prove this by show that set of states that satisfy $grow_1$ and $grow_2$. 

 If a state $\vec{s}$ satisfies $grow_1$ in $(k+1)^{th}$ iteration when the input system is $M$ then all its successors were 
 added to $Y$ in $i^{th}$ such that $i \leq k$. By induction hypothesis when the input machine is $M_T$, 
 all successors of $\vec{s}$ will added to $Y$ before $(k+1)^{th}$ iteration as $\vec{s}$ has same set of successors in both $M$ and $M_T$.
 Hence $\vec{s}$ will satisfy $grow_1$ in  $(k+1)^{th}$ iteration.

If a state $\vec{s}$ satisfies $grow_2$ in $(k+1)^{th}$ iteration when the input system to the algorithm is $M$, 
then on ignoring the states that are already added to $Y$, there exists only one trace 
$\vec{s}, \vec{s_1}, \vec{s_2}, \dots, \vec{s_n}$ starting from $\vec{s}$ such that $\vec{s_n}$ satisfies $grow_1$. The same trace also exists
when input system is $M_T$ as $M_T$ preserves all traces in $M$, set of states satisfying $grow_1$ is same and
set of state already added to $Y$ is also same in both cases. 
Also there cannot be any additional trace starting from $\vec{s}$ as it will contradict the fact that $M_T$ preserves 
all traces. Hence $\vec{s}$ will also satisfy $grow_2$ in $(k+1)^{th}$ iteration when the input system to the 
algorithm is $M_T$. Note that we assume $\mathit{pre^*}$ queries used to compute the formula for  
$grow_2$ will terminate on both $M$ and $M_T$.

Hence the theorem lemma statement holds for all values of $n$. 
 \end{proof}
 
 \begin{theorem}
 \label{thm:trace_flattable_systems2}
 Given a trace flattable counter system $M$ a property $\eglobally{\phi}$ Algorithm~$\computeGlobalOverName$ will terminate
 if the $\mathit{pre^*}$ queries terminate.
 \end{theorem}
 \begin{proof}
 	The proof follows from the proof of Lemma~\ref{thm:trace_flattable_systems1} and Lemma~\ref{thm:flat_systems}.
 \end{proof}
 
 \begin{theorem}
 \label{thm:over_approx_characterization}
 Given any property $\eglobally{\phi}$ Algorithm  $\computeGlobalOverName$ will terminate on a systems $M$ if:\\ 
 (a) all $\mathit{pre}^*$ queries on the system $M_1$ terminate, where $M_1 = = \refineSystem{M}{\phi}$\\
 (b) there exists an integer bound k, and a (finite or infinite) set of flattenings of M1 such that each flattening 
 N in the set contains at most k simple cycles (each one involving an arbitrary number of control states), 
 and such that each trace in M1 that starts from a state that does not satisfy $\eglobally{\phi}$ is exhibited by at least one of the 
 flattenings mentioned above.
 \end{theorem}
 \begin{proof}
 We provide only the sketch of the proof. The detailed proof is part of ongoing work.
 It follows from the proof of Theorem~\ref{thm:flat_systems} that given any flat system Algorithm $\computeGlobalOverName$ will terminate 
 in finite number of iteration of the loop in the algorithm. The number of iterations of the loop required to terminate 
 is a function of number of simple cycles in the given counter system. Given a set of flat systems $S$ the algorithm will require
 maximum of $k$ iteration where $k$ is maximum number of simple cycles in any flat system that belongs to $S$. Hence
 if there is integer bound on number of simple cycles in any flat system in the set $S$ then the algorithm will definitely terminate on 
 combined counter system formed by considering all the flat systems in $S$ together.
 
 If there is a set of flattenings $N_S$ of $M_1$ such that all traces from states that do not satisfy $\eglobally{\phi}$ are preserved then
 set of states that do not satisfy $\eglobally{\phi}$ in $M_1$ will definitely not satisfy the property $\eglobally{\phi}$ in $N_S$. By argument
 given above algorithm will definitely terminate on counter system formed by combining all flattening in $N_S$ together. It can be shown
 using induction that the number of iterations of the loop in Algorithm $\computeGlobalOverName$ required to terminate on combined system 
 formed from $N_S$ and $M_1$ is same and hence algorithm will terminate on $M_1$ under the given assumptions.
 \end{proof}


==> secGlobalUnderThmFME.tex <==
\subsection{Theoretical claims}
\label{ssec:under-approx-thms}
% 
% Theorem~\ref{thm:compute-global-correctness}, Theorem~\ref{thm:precision} and Lemma~\ref{thm:under_approx} prove correctness and precision characteristics  of 
% Algorithm~\ref{algo:under_approx}, both when it terminates and when forced to terminate. 
% 
% \begin{theorem}
% \label{thm:compute-global-correctness}
% Given a counter system $M=\langle Q,C,\Sigma,\phiinit,G,F\rangle$, the set of states that satisfy the formula $\eglobally{\phi}$ in $M$ is precisely given by the set of
% states that satisfy the formula $\forall k\geq 0.\ \prek{M_1}{\phi}$, where $M_1=\refineSystem{M}{\phi}$.
% \end{theorem}
% Note that the set of states that satisfy the property $\eglobally{\phi}$ in the counter system $M$ and $M_1$ are the same, where $M_1$ is a refinement of $M$ with respect to 
% $\phi$. This is because of the fact that the traces from $\phi$ that are exhibited by the counter systems $M$ and $M_1$ are same. Therefore for the rest of this section we 
% prove the precision and termination characteristics of Algorithm~\ref{algo:under_approx} are proved on the the counter system $M_1$.
% \begin{theorem}
% \label{thm:precision}
% Given a counter system $M$ and a set of states $\phi$, Algorithm~\ref{algo:under_approx} returns precisely the set of states that 
% satisfy $\eglobally{\phi}$ in $M_1$ whenever it terminates, where $M_1=\refineSystem{M}{\phi}$.
% \end{theorem}
% 
% \begin{theorem}\label{thm:under_approx}
%  Given a counter system $M$ and a set of states $\phi$, Algorithm~\ref{algo:under_approx} returns an under-approximation of the set of states that satisfy $\eglobally{\phi}$
% in the counter system $M_1$ when prematurely terminated, where $M_1=\refineSystem{M}{\phi}$.
% \end{theorem}

It is not very difficult to see that the set $X$ maintained by the algorithm is a  monotonically non-decreasing 
under-approximation of the set of states that satisfy $\eglobally{\phi}$ in $M$. Also, that upon termination the accumulated set $X$ contains the precise solution. However, it is \emph{not} necessarily true that in all cases where $X$ becomes equal to the precise solution the algorithm will detect this situation and terminate. 

A sufficient condition for the termination of the algorithm on a system $M$ is that (a) $\mathit{pre}^k$ and $\mathit{pre}^*$ queries terminate on flattenings of the refined system $M_1$, and (b)
the system $M_1$ $\equiv$ $\refineSystem{M}{\phi}$ has a flattening $N$ such that $\traces{N}{\phi-X}=\traces{M_1}{\phi-X}$, where $X$ is the set of states that satisfy $\eglobally{\phi}$ in $N$.

While this is a simple condition to state, it actually under-approximates the cases on which the algorithm terminates, because the algorithm actually uses the accumulated set $X$ in its termination check. Yet, this characterization describes a class that's strictly broader than the class addressed by the approach of Demri et al.~\cite{dem2006}, which targets only the class of systems $M$ that are trace-flattable wrt $\phiinit$; i.e., $M$ needs to have a flattening $N$ such that $N$ exhibits \emph{all} traces that $M$ exhibits from \emph{all} states that are reachable in $M$.

We provide formal statements and
proofs of all our claims in Appendix~\ref{ssec:under-approx-thms-proof}.

%% Algorithm~\ref{algo:under_approx} will return precise reults on all systems %% whenever it terminates and under-approximates the set of states that %% satisfy $\eglobally{\phi}$.
%% Let $N$ be a given counter system and $M_1$ be the refinement of $M$ wrt to %% $\phi$. Let $X$ be the set of states that satisfy $\eglobally{\phi}$ in %% $M_1$.
%% If $N$ is a flattening of $M_1$ such (a)that every state that 
%% satisfies $\eglobally{\phi}$ in $M_1$ satisfies $\eglobaselly{\phi}$ in $N$ %% and (b) $\traces{N}{\phi-X}=\traces{M_1}{\phi-X}$, then %% Algorithm~\ref{algo:under_approx} terminates.
%% These results are easy to see and are proved formally in our technical %% report~\cite{techReport}.
%% % of it
%% % Theorem~\ref{thm:charaterization} defines a class of systems on which %% under-approximation is guaranteed to terminate and return 
%% % precise results. 
%% Corollary~\ref{lemma:trace-flattable-termination} proves that %% Algorithm~\ref{algo:under_approx} approach terminates on all
%% trace-flattable systems~\cite{dem2006}.

% \begin{theorem}
% \label{thm:charaterization}
% Given a counter system $M$, let $M_1$ be the refinement of $M$ with respect to to $\phi$.
% Let $X$ be the set of states that satisfy $\eglobally{\phi}$ in $M$.
% Algorithm~\ref{algo:under_approx} terminates if
% and only if (a) there exists a flattening $N$ of $M_1$
% such that every state that satisfies $\eglobally{\phi}$ in $M$ has at least one infinite trace in $N$ and 
% (b) the systems $M_1$ and $N$ are trace equivalent with respect to the set of states 
% that do not satisfy $\eglobally{\phi}$ that is $\traces{M_1}{\phi-X}=\traces{N}{\phi-X}$.
% \end{theorem}

%% \begin{corollary}
%% \label{lemma:trace-flattable-termination}
%% The class of systems on which our approach terminates, is a strict super %% set of the class of systems that are 
%% trace-flattable with respect to $\phiinit$.
%% % Given a counter system $M$, if $M$ is trace flattable then the routine %% $\mathit{compute}$-$\mathit{Global}$ definitely terminates 
%% % for any given $\phi$, i.e, the class of systems that the routine %% $\computeGlobalName$ terminates is a strict superset of
%% % trace-flattable systems.
%% \end{corollary}
%% We provide an outline of the proof of %% Corollary~\ref{lemma:trace-flattable-termination}. 
%% Given a system $M$, let $X$ is the set of reachable states that definitely 
%% satisfy $\eglobally{\phi}$ in $M$ as computed by %% Algorithm~\ref{algo:under_approx}. If $M$ is trace-flattable, then there %% exists a flattening $N$ of $M$ such that 
%% $\traces{M}{\phiinit}=\traces{N}{\phiinit}$. Since %% Algorithm~\ref{algo:under_approx} explores all flattenings in a breadth %% first manner, it will find this flattening $N$. 
%% The inital pre-pass ensures that the set of states $\phi-X$ is a subset of %% $\phireach$ and hence the flattening $N$ will preserve all traces from %% $\phi-X$.
%% % The flattening $N$ also falls in the characterization stated in %% Theorem~\ref{thm:charaterization} because $\phi-X$ is a subset of reachable %% states and hence all traces from
%% % $\phi-X$ that are in $M$ are also present in $N$. 
%% Therefore Algorithm~\ref{algo:under_approx} will terminate on all %% trace-flattable systems.


%% Note that the characterization that we state is on the system $M_1$. $M_1$ %% is the refinement of $M$ with respect to $\phi$. 
%% The formula $\phi$ which represents a set of states is dependent on the %% temporal property that is provided as the input. 
%% Therefore the characterization we state is dependent on the system and the 
%% temporal property. But if the system $M$ is trace-flattable then %% under-approximation approach terminates for \emph{any} given formula %% $\phi$. 



==> secGlobalUnderThmTR.tex <==
%\subsubsection{Correctness, precision and termination characteristics of under- approximation approach:\\}
\label{ssec:under-approx-thms-proof}
In this section we give the formal statements and the proofs of the various claims of Algorithm~$\computeGlobalUnderName$ in Section~\ref{sec:under-approx}.


Theorem~\ref{thm:compute-global-correctness}, Theorem~\ref{thm:precision} and Lemma~\ref{thm:under_approx} prove correctness and precision characteristics  of 
Algorithm~$computeGlobalUnderName$, both when it terminates and when forced to terminate. 

\begin{theorem}
\label{thm:compute-global-correctness}
Given a counter system $M=\langle Q,C,\Sigma,\phiinit,G,F\rangle$, the set of states that satisfy the formula $\eglobally{\phi}$ in $M$ is precisely given by the set of
states that satisfy the formula $\forall k\geq 0.\ \prek{M_1}{\phi}$, where $M_1=\refineSystem{M}{\phi}$.
\end{theorem}
\begin{proof}
Let $M_1$ be the refined system returned by
$\refineSystem{M}{\phi}$.  Let $\vec{s}$ be a state in $M$ which is reachable from $\phiinit$.
Let $\vec{s}\models\eglobally{\phi}$.

\begin{flalign}
\label{eqn:globalForward}
&\vec{s}\models\eglobally{\phi}&\nonumber\\
%\implies &\exists \vec{s_1},\vec{s_2},\dots.\,
%\forall i\geq 1.\, \exists a_i \in \Sigma.\, \vec{s_i}\models g_{a_i}\wedge 
%f_{a_i}(\vec{s},\vec{s_{i+1}}) \wedge \vec{s_i}\models\psi_1 \wedge \vec{s}
%= \vec{s_1} &\nonumber\\
\implies &\exists \vec{s_1},\vec{s_2},\dots.\,
\forall i\geq 1.\, \exists a \in \Sigma.\, \vec{s_i}\models g_{a}\wedge 
f_{a} \wedge \vec{s_i}\models\phi \wedge \vec{s}=\vec{s_1}&\nonumber\\
\implies &\forall k\geq 0.\, \exists \vec{s_1},\vec{s_2},\dots,\vec{s_k}.\,\forall i, 1\leq i< k.\, 
 (\exists a \in \Sigma.\, \vec{s_i}\models (g_{a} \wedge  \phi)\wedge &\nonumber\\ 
& f_{a})\wedge \vec{s_k} \models \phi \wedge 
\vec{s} = \vec{s_1}
\end{flalign}
Since $M_1$ is a refinement of $M$ with respect to $\phi$
$g_{a_1}=g_{a}\wedge\phi$ and $f_{a_1}=f_{a}$ are the guards and actions of the refined system, Equation~\ref{eqn:globalForward} can be rewritten as
\begin{flalign*}
&\forall k\geq 0.\, \exists \vec{s_1},\vec{s_2},\dots,\vec{s_k}.\,\forall i, 1\leq i< k.\, 
 (\exists a_1 \in \Sigma_1.\, \vec{s_i}\models g_{a_1} \wedge &\nonumber\\ 
 & f_{a_1})\wedge \vec{s_k} \models \phi \wedge 
\vec{s} = \vec{s_1}\\
&\implies \vec{s}\models\forall k\geq 0.\, \prek{M_1}{\phi}&
\end{flalign*}


The converse of the theorem can be proved as follows:
Let $\vec{s}$ satisfy $\phi \equiv \forall k\geq
0.\ \prek{M_1}{\phi}$. Let $\vec{s}$ be reachable.
\begin{flalign*}
\implies &\forall k\geq0.\,\, \exists \vec{s_1},\vec{s_2},\dots,\vec{s_k}.\, \forall i, 1\leq i< k.\, 
(\exists a_1 \in \Sigma_1.\, \vec{s_i}\models g_{a_1}\wedge &\\ 
& f_{a_1})\wedge \vec{s_k} \models \phi \wedge 
\vec{s} = \vec{s_1}&\\
\implies &\exists \vec{s_1},\vec{s_2},\dots.\, \forall i\geq 1.\, 
(\exists a_1 \in \Sigma_1.\, \vec{s_i}\models g_{a_1}\wedge
f_{a_1} \wedge \vec{s_i}\models\phi) \wedge 
\vec{s} =\vec{s_1}&\\
&\mbox{[ By K\"{o}nig's Lemma\footnotemark[2] ]}&\\
\implies &\exists \vec{s_1},\vec{s_2},\dots.\, \forall i\geq 1.\, 
(\exists a \in \Sigma.\, \vec{s_i}\models g_{a}\wedge
f_{a}) \wedge \vec{s_i}\models\phi) \wedge 
\vec{s} =\vec{s_1}&\\
\implies &\vec{s}\models \eglobally{\phi}&
\end{flalign*}
\end{proof}



Note that the set of states that satisfy the property $\eglobally{\phi}$ in the counter system $M$ and $M_1$ are the same, where $M_1$ is a refinement of $M$ with respect to 
$\phi$. This is because of the fact that the traces from $\phi$ that are exhibited by the counter systems $M$ and $M_1$ are same. Therefore for the rest of this section we 
prove the precision and termination characteristics of Algorithm~$computeGlobalUnderName$ are proved on the the counter system $M_1$.
\begin{theorem}
\label{thm:precision}
Given a counter system $M$ and a set of states $\phi$, Algorithm~$computeGlobalUnderName$ returns precisely the set of states that 
satisfy $\eglobally{\phi}$ in $M_1$ whenever it terminates, where $M_1=\refineSystem{M}{\phi}$.
\end{theorem}
\begin{proof}
 Let $X$ be a Presburger formula representing a set of states in the counter system $M_1$, returned by 
Algorithm~$computeGlobalUnderName$ upon termination. \\
\textbf{Claim A:} Consider a state $\vec{s}\in X$.
% then $\vec{s} \models \eglobally{\phi}$ in the counter system $M$.
We will prove that $\vec{s}\models \forall k\geq 0.\ \prek{M_1}{\phi}$ where $M_1$ is a refinement of $M$ with respect to to $\phi$.
Then by Theorem~\ref{thm:compute-global-correctness}, it follows that $\vec{s}\models\eglobally{\phi}$ in the counter system $M$.

Let $N$ be some flattening of $M_1$ that was produced by Algorithm~$computeGlobalUnderName$ prior to termination. Then,
$\vec{s}\in X$\\
$\implies \vec{s}\in\forall k\geq 0.\ \prek{N}{\phi}$.
Since $N$ is a flattening of $M_1$, $\traces{N}{\phi}\subseteq\traces{M_1}{\phi}$. Therefore every state which satisfies 
$\forall k\geq 0.\ \prek{N}{\phi}$ will satisfy $\forall k\geq 0.\ \prek{M_1}{\phi}$.\\
$\implies \vec{s}\models \forall k\geq 0.\ \prek{M_1}{\phi}$.\\
Then by Theorem~\ref{thm:compute-global-correctness},
$\vec{s}\models\eglobally{\phi}$ in the counter system $M$.

\textbf{Claim B:} If a state $\vec{s}\notin X$ then $\vec{s}\not\models \eglobally{\phi}$ in $M$.\\
Let $N$ be the final flattening of $M_1$ that was analysed when the algorithm terminated.
$\vec{s}\notin X$\\
$\implies \vec{s}\notin\forall k\geq 0.\ \prek{N}{\phi}$.
Therefore by definition of $\forall k\geq 0.\ \prek{N}{\phi}$ there is no infinite length path in $N$ 
starting from $\vec{s}$. Now since $\vec{s}\notin X$, and we terminate only when
$\traces{M_1}{\phi-X}=\traces{N}{\phi-X}$ it follows that there is no infinite length path in 
$M_1$ from the state $\vec{s}$. Then by theorem~\ref{thm:compute-global-correctness} $\vec{s}\not\models \eglobally{\phi}$ 
in the counter system $M$.
\end{proof}

\begin{theorem}\label{thm:under_approx}
 Given a counter system $M$ and a set of states $\phi$, Algorithm~$computeGlobalUnderName$ returns an under-approximation of the set of states that satisfy $\eglobally{\phi}$
in the counter system $M_1$ when prematurely terminated, where $M_1=\refineSystem{M}{\phi}$.
\end{theorem}

\begin{proof}
The proof follows directly from Claim A in the proof of Theorem~\ref{thm:precision}.
 %\qed
\end{proof}

Theorem~\ref{thm:charaterization} defines a class of systems on which under-approximation is guaranteed to terminate and return 
precise results. Corollary~\ref{lemma:trace-flattable-termination} proves that under-approximation approach terminates on all
trace-flattable systems~\cite{dem2006}.

\begin{theorem}
\label{thm:charaterization}
Given a counter system $M$, let $M_1$ be the refinement of $M$ with respect to to $\phi$.
%Let $X$ be the set of states that satisfy $\eglobally{\phi}$ in $M$.
Algorithm~$\computeGlobalUnderName$ terminates if 
(a) $\mathit{pre}^k$ and $\mathit{pre}^*$ queries terminate on the flattenings on $M_1$ and
(b) there exists a flattening $N$ of $M_1$ such that $\traces{M_1}{\phi-X}=\traces{N}{\phi-X}$ where $X$ is the set of states that satisfy the $\eglobally{\phi}$ in $N$.
%such that every state that satisfies $\eglobally{\phi}$ in $M$ has at least one infinite trace in $N$ and 
%(b) the systems $M_1$ and $N$ are trace equivalent with respect to the set of states 
%that do not satisfy $\eglobally{\phi}$ that is $\traces{M_1}{\phi-X}=\traces{N}{\phi-X}$.
\end{theorem}
\begin{proof}
Let $N$ be a flattening of $M_1$ such that $M_1$ and $N$ are such that $\traces{M_1}{\phi-X}=\traces{N}{\phi-X}$.
Since $X$ is the set of states that satisfies $\eglobally{\phi}$ in $N$, there exists an infinite trace from every state in $X$ in $N$.
Since there is at least one infinite trace from every state $\vec{s}$ in $X$ in the counter system $N$,
$\vec{s}\in\ \forall k\geq 0.\ \prek{N}{\phi}$. Since the $\mathit{pre}^*$ and $\mathit{pre}^k$ queries terminate on every flattening $N$ of $M_1$, the routines 
$\prek{N}{\phi}$ and the trace equivalence
check in Lines~\ref{line:expand_X} and \ref{line:trace-flattening-check} in Algorithm~$computeGlobalUnderName$ will terminate. 
Also traces $N$ $\traces{N}{\phi-X}=\traces{M_1}{\phi-X}$. Therefore the trace flattening check will return $\tru$ and hence algorithm will
terminate. The only thing that remains to prove is that we will definitely find such a flattening $N$ if it exists.
Note that we explore different flattenings of increasing lengths in a breadth first manner. Since $N$ is a flattening of $M_1$,
$N$ is of finite length and hence breadth first generation of flattenings (in Line ~\ref{line:gen_flat}) will find it. This is because the there will be no previous flattenings on which
$\mathit{pre}^k$ and $\mathit{pre^*}$ will go into non-termination.
\end{proof}


We say that a system $M$ is \emph{trace flattable} if there is a flattening $N$ of $M$ such that $\traces{M}{\phiinit}=\traces{N}{\phiinit}$.
To prove that Algorithm $\computeGlobalUnderName$ terminates on trace flattable systems, 
we make an assumption about the given system $M$ for both this approach and for the subsequently presented over-approximation approach: that all its guards contain
$\phireach$ as a conjunct, where $\phireach$ is the set of reachable states
in $M$. This is to restrict our algorithms from analyzing states that are
not reachable in $M$.
\begin{corollary}
\label{lemma:trace-flattable-termination}
The class of systems on which our approach terminates, namely the class identified in Theorem~\ref{thm:charaterization}, is a strict super set of the class of trace-flattable systems.
% Given a counter system $M$, if $M$ is trace flattable then the routine $\mathit{compute}$-$\mathit{Global}$ definitely terminates 
% for any given $\phi$, i.e, the class of systems that the routine $\computeGlobalName$ terminates is a strict superset of
% trace-flattable systems.
\end{corollary}
\begin{proof}
If the system $M$ is trace-flattable then there exists a flattening $N$ of $M$ such that 
$\traces{M}{\phiinit}=\traces{N}{\phiinit}$. Let $X$ be the set of reachable states that satisfy $\eglobally{\phi}$
in the counter system $M$. Due to trace equivalence, it follows that $X$ precisely represents the set of states that
satisfy $\eglobally{\phi}$ in $M$. Also from trace equivalence it follows that $\traces{M}{\phi-X}=\traces{N}{\phi-X}$. Therefore 
Algorithm~$\computeGlobalUnderName$ will definitely terminate when it generates the flattening $N$ with the precise answer $X$.
The generation of $X$ is guaranteed as per Theorem~\ref{thm:charaterization} (Note that the algorithm may terminate even before 
the system $N$ is generated). 
\end{proof}



Note that the characterization that we state is on the system $M_1$. $M_1$ is the refinement of $M$ with respect to $\phi$. 
The formula $\phi$ which represents a set of states is dependent on the temporal property that is provided as the input. 
Therefore the characterization we state is dependent on the system and the 
temporal property. But if the system $M$ is trace-flattable then under-approximation approach terminates for \emph{any} given formula $\phi$. 


